Flexible Control Flow Graph Alignment for Delivering Data-Driven Feedback to Novice Programming Learners

Supporting learners in introductory programming assignments at scale is a necessity. This support includes automated feedback on what learners did incorrectly. Existing approaches cast the problem as automatically repairing learners' incorrect programs extrapolating the data from an existing correct program from other learners. However, such approaches are limited because they only compare programs with similar control flow and order of statements. A potentially valuable set of repair feedback from flexible comparisons is thus missing. In this paper, we present several modifications to CLARA, a data-driven automated repair approach that is open source, to deal with real-world introductory programs. We extend CLARA's abstract syntax tree processor to handle common introductory programming constructs. Additionally, we propose a flexible alignment algorithm over control flow graphs where we enrich nodes with semantic annotations extracted from programs using operations and calls. Using this alignment, we modify an incorrect program's control flow graph to match the correct programs to apply CLARA's original repair process. We evaluate our approach against a baseline on the twenty most popular programming problems in Codeforces. Our results indicate that flexible alignment has a significantly higher percentage of successful repairs at 46% compared to 5% for baseline CLARA. Our implementation is available at https://github.com/towhidabsar/clara.

==> background.tex <==
\section{Background}
\label{sec:background}

A program's control flow represents the order in which its statements are evaluated. Conditional or loop statements like \texttt{if} or \texttt{while} modify such a flow. In Figure~\ref{fig:correct-killer}, lines 4 and 5 are executed in sequence; however, the execution of line 6 depends on the statement in line 5 evaluating to true. A control dependency models immediate control flow information. Data dependencies model the possible set of origins that each variable in a given statement may take. In Figure~\ref{fig:correct-killer}, the value of \texttt{x} in line 3 can be equal to zero since it is initialized in line 2, or more than zero because \texttt{x} is updated in line 7 and, in line 3, it is evaluated again (loop).

A program dependence graph $G = (V, E, l_s, l_e)$ of a program $p$ is a directed, labeled multigraph, where $V$ is a set of nodes representing statements in $p$, $E: V \times V$ is a set of directed edges, $l_s: V \rightarrow (L_s, m)$ is a node labeling function, and $l_e: E \rightarrow \{Ctrl, Data\}$ is an edge labeling function. Let $(v_s, v_t) \in E$, $l_e((v_s, v_t)) = Ctrl$ indicates that the execution of node $v_t$ depends on node $v_s$ evaluating to true; furthermore, $l_e((v_s, v_t)) = Data$ represents that $v_t$ uses a variable declared or re-assigned by $v_s$. $L_s$ contains labels that summarize the semantics of a program statement, such as $Assign$, $Call$, and $Ctrl$ to denote variable assignments, calls to other methods, and condition or loop statements, respectively. In addition, $L_s$ includes labels to represent operation semantics and constants of a program statement, which include $Acc$, $Add$, and $Sub$ to encode array access, addition, and substraction, respectively. Since a program statement may contain multiple operations that are the same, e.g., multiple array accesses, $m: L_s \rightarrow \mathbb{N}$ is a function to support multisets. Note that, for the sake of simplicity, we omit the details of multi-method program dependence graphs, i.e., programs that contain multiple methods. In such cases, we extend $L_s$ and $\{Ctrl, Data\}$ allowing nodes denoting method entry points, method calls, and parameters and result of a method call~\cite{DBLP:conf/icse/HorwitzR92}. In Figure~\ref{fig:pdg-align-killer}, $u_3$ is obtained from line 3 in Figure~\ref{fig:correct-killer}, i.e., \texttt{while (x < a.length)}; $l_s(u_3) = \{Ctrl, Lt, length\}$ since it is a loop statement, is checking \texttt{x} is less than \texttt{a.length}, and it is accessing the length of the array. Line 3 directly controls its execution (loop) and the execution of lines 4, 5 and 7, which results in the following control dependency edges: $l_e((u_3, u_3)) = l_e((u_3, u_4)) = l_e((u_3, u_5)) = l_e((u_3, u_7)) = Ctrl$. Since it is using variable \texttt{x}, there is a data dependency coming from line 7, which is updating such variable, i.e., $l_e((u_7, u_3)) = Data$.

Let $G_1 = (V_1, E_1)$ and $G_2 = (V_2, E_2)$ be two directed graphs such that $|V_1| \leq |V_2|$. Subgraph isomorphism consists of finding all non-induced solutions $\phi: V_1 \rightarrow V_2$ such that $\forall (u_i, u_j) \in E_1 \Rightarrow (\phi(u_i), \phi(u_j)) \in E_2$. Note that, if we take labels into account, $\phi(u_i) = v_j$ if and only if the labels of $u_i$ are included or equal to the labels of $v_j$. A solution $\phi: V_1 \rightarrow V_2$ is induced if it is non-induced and $\forall (u_i, u_j) \notin E_1 \Rightarrow (\phi(u_i), \phi(u_j)) \notin E_2$. In general, subgraph isomorphism assumes that $|V_1| \ll |V_2|$; furthermore, it computes exact matches, i.e., $G_1$ needs to be exactly contained in $G_2$. The problem of approximate graph alignment consists of finding an injective function $\varphi: V_1 \rightarrow V_2$ such that $|V_1| \leq |V_2|$. This problem is a relaxation of the subgraph isomorphism problem in which we assume that $|V_1| \approx |V_2|$, and $G_1$ is approximately contained in $G_2$. 

==> framework.tex <==
\section{Flexible program alignment}
\label{sec:discover}

Assume an incorrect program that we wish to analyze with respect to an existing correct program. We transform both programs into program dependence graphs and align them using approximate graph alignment (Section~\ref{subsec:aligning}). To discover repair suggestions, our goal is to analyze the alignment pairs that are significantly different, which entails replacing incorrect by correct statements. Depending on the size of the aligned graphs, we also analyze non-aligned statements that are appealing to be added or removed (Section~\ref{subsec:repairing}).

\subsection{Aligning program dependence graphs}
\label{subsec:aligning}

We wish to compute an alignment between the statements in a correct program with respect to the statements in an incorrect program. The computation of such an alignment takes topological and semantic information into account. On one hand, topological information encodes the context of each statement regarding its control and data dependencies, i.e., what are the statements that must be fulfilled in order for a given statement to be executed, and what are the variable uses of such a statement. On the other hand, semantic information allows us to distinguish statements that are performing different operations, such as addition or an API call. Let $G_1 = (V_1, E_1, l^1_s, l^1_e)$ and $G_2 = (V_2, E_2, l^2_s, l^2_e)$ be two program dependence graphs. At this stage, we are agnostic to correctness and incorrectness of the programs evaluated, so $G_1$ can be either correct (and $G_2$ is then incorrect), or incorrect (and $G_2$ is then correct). Our first goal consists of computing all the pairwise similarities between nodes in $V_1$ and $V_2$. The similarity of nodes $u_i \in V_1$ and $v_j \in V_2$ is measured as follows~\cite{DBLP:journals/pvldb/KhanWAY13, Kuchaiev1341, DBLP:conf/kdd/ZhangT16}: $Sim(u_i, v_j) = \alpha \, Top(u_i, v_j) + (1 - \alpha) \, Sem(u_i, v_j)$, where $Top$ and $Sem$ are topological and semantic similarities, respectively, and $\alpha \in [0, 1]$ is a parameter to balance the contribution of each type of similarity. $Sim(u_i, v_j) = 1$ entails that both nodes are identical, while $Sim(u_i, v_j) = 0$ implies that nodes $u_i$ and $v_j$ are completely dissimilar.

\begin{figure}
\centering
\includegraphics[scale=0.73]{graphlets.pdf}
\caption{Directed graphlets that contain two and three nodes along with their orbits (non-symmetric nodes)}
\label{fig:graphlets}
\end{figure}

We rely on graphlets to compute $Top(u_i, v_j)$, which are all possible connected, directed graphs of up to a number of nodes~\cite{Kuchaiev1341}. Given a node $u$ in a certain graph $G$, the signature of $u$, denoted as $s_n(u)$ where $n \in \mathbb{N}$, is computed by finding induced solutions for all graphlets, and counting the number of unique nodes that are mapped to $u$. The signature must contain unique values, so we focus on orbits, i.e., non-symmetric nodes in a given graphlet; as a result, $s_n$ corresponds to orbit $o_n$. Figure~\ref{fig:graphlets} shows two- and three-node, directed graphlets. Note that $s_0$ and $s_1$, respectively derived from $o_0$ and $o_1$, correspond to the in-degree and out-degree of a given node, e.g., in Figure~\ref{fig:pdg-align-killer}, $s_0(u_3)=3$ and $s_1(u_3)=1$ (ignoring self-edges that we discuss below). In addition, $s_2(u_3)=0$ since there are two subgraphs resembling this graphlet, i.e., $\{(u_3, u_4), (u_7, u_4)\}$ and $\{(u_3, u_5), (u_7, u_5)\}$; however, they are not induced because of the existence of $(u_7, u_3)$. We also have that $s_3(u_3)=0$ since there are no incoming edges, and $s_4(u_3)=2$, which corresponds to the following subgraphs: $\{(u_3, u_5), (u_5, u_6)\}$ and $\{(u_3, u_7), (u_7, u_6)\}$.

We do not consider graphlets with self-edges as it exponentially increases its total number. Therefore, for every self-edge $(u_i, u_i) \in E$ such that $l_e((u_i, u_i)) = Ctrl$, we remove such edges from the graph and add a $Loop$ label to $l_s(u_i)$ to indicate that the node is representing a loop statement, which implies that loops will be solely considered in the semantic similarity. Furthermore, we discard self-edges such that $l_e((u_i, u_i)) = Data$, which are typically considered in the semantic similarity by different labels, such as $PostIncr$ (post-increment operator) or $PreDecr$ (pre-decrement operator). Additionally, we do not take edge labels, $Ctrl$ and $Data$, into account and consider the whole graph for topology purposes. Another choice would be to split program dependence graphs into control dependence and data dependence graphs. However, control dependence and data dependence graphs may be disconnected, e.g., a \texttt{break} (labeled or unlabeled) or a \texttt{return;} (note the semicolon) statements are disconnected nodes in a data dependence graph.

Once node signatures have been computed, the topological similarity between nodes $u_i$ and $v_j$ is computed as follows~\cite{Kuchaiev1341}:

\begin{align*}
Top(u_i, v_j) = 1 - \dfrac{\sum\limits_{n} w_n\,\dfrac{|log(s_n(u_i)+1)-log(s_n(v_j)+1)|}{log(max\{s_n(u_i), s_n(v_j)\}+2)}}{\sum\limits_{n} w_n}
\end{align*}

\noindent where $w_n$ represents a weight that takes the dependencies between orbits in graphlets into account, and $s_n(u_i)$ and $s_n(v_j)$ denote the signatures of nodes $u_i$ and $v_j$, respectively. The logarithm function avoids large values of $s_n$ to dominate topological similarities.

The semantic similarity of nodes $u_i$ and $v_j$ is computed as follows: $Sem(u_i, v_j) = Jac(l_s(u_i), l_s(v_j))$, where $Jac$ computes the Jaccard similarity between the two multisets of labels~\cite{DBLP:journals/prl/Kosub19}. For instance, in Figure~\ref{fig:pdg-align-killer}, $Sem(u_3, v_3) = 1$ and $Sem(u_3, v_4) = .5$. Note that there are more sophisticated methods to compute such a semantic similarity, e.g., defining similar operations or API calls~\cite{DBLP:conf/icse/KimKBC0KT18}.

We compute similarities $Sim(u_i, v_j)$ for every pair of nodes $u_i \in V_1$ and $v_j \in V_2$. The next step consists of computing an alignment between both graphs, i.e., $\varphi: V_1 \rightarrow V_2$ ($|V_1| < |V_2|$). Kuchaiev et al.~\cite{Kuchaiev1341} propose a neighborhood-based method to compute such an alignment: node pairs are greedily selected based on their neighborhoods. The method works as follows: 1)~Find a pair seed $(u_i, v_j)$ that has not been aligned yet such that $Sim(u_i, v_j)$ is maximum; 2)~Find all neighbors of $u_i$ and $v_j$ within radius $r$, and select the pairs with the maximum node similarity; 3)~Increase $r$ until there are no more neighbors of $u_i$ or $v_j$ to consider; and 4)~Repeat the process until all nodes in $V_1$ are aligned. This neighborhood-based method does not guarantee an optimal alignment, i.e., there can be other alignments for which the sum of node similarities are higher than the alignment output by this method. However, the method guarantees that nodes that are direct or indirect neighbors in one graph are aligned with nodes that are direct or indirect neighbors in the other graph. Since we rely on node similarities for discovering repairs, we use a similarity-based method that provides the opposite guarantees: it computes optimal alignments but does not guarantee that neighborhood is preserved. Note that node similarities encode neighborhood information based on graphlets, so our method takes into account node pairs whose signatures are similar and, therefore, their neighborhoods are approximately similar.

We cast the problem of finding an alignment as finding a maximum weight matching in bipartite graphs. Let $B = (V_1, V_2, E, \omega)$ be a bipartite graph where $V_1$ and $V_2$ are the sets of nodes of $G_1$ and $G_2$ ($V_1 \cap V_2 = \emptyset$), respectively, $E: V_1 \times V_2$ is a set of undirected edges, and $\omega: E \rightarrow \mathbb{N}$ is a function that assigns weights to the edges as follows: $\omega(u_i, v_j) = Sim(u_i, v_j)$. There are several algorithms in the literature to compute maximum weighted matchings that find augmenting paths that alternatively connect edges in $V_1$ and $V_2$, ensuring that the final similarity weight is maximized and, thus, producing the alignment $\varphi$ with maximum similarity~\cite{DBLP:journals/tcs/Sankowski09}. In Figure~\ref{fig:pdg-align-killer}, our similarity-based method produces the following alignment shown as double-headed arrows: \{$\varphi(u_3) = v_3$, $\varphi(u_4) = v_6$, $\varphi(u_5) = v_4$, $\varphi(u_6) = v_5$, $\varphi(u_7) = v_7$\}. The statements mapped by $\varphi$ correspond to statements that perform similar computations.

\subsection{Discovering repair suggestions}
\label{subsec:repairing}

Once we have computed an alignment $\varphi : V_1 \rightarrow V_2$ between two program dependence graphs $G_1$ and $G_2$, our goal is to discover repair suggestions, i.e., statements in the correct program that can be used to fix the incorrect program. To discover these statements, we rely on the node similarities of the pairs available in the approximate graph alignment $\varphi$. Recall that approximate graph alignment assumes that $|V_1| \leq |V_2|$, which leads to two different situations:

\begin{enumerate}
\item If $G_1$ is correct and $G_2$ is incorrect, non-aligned nodes belong to the incorrect program and we aim to remove them. This is the case of superfluous/inadequate statements.
\item Otherwise, non-aligned nodes belong to the correct program and we aim to add them to the incorrect program. This is the case of missing statements.
\end{enumerate}

Programs in Figures~\ref{fig:correct-killer} and~\ref{fig:incorrect-killer} are an example of the former situation since the first one is correct and smaller than the second one, which is incorrect. In such a case, we aim to remove lines 8 and 9 from the incorrect program.

First, we address the problem of finding replacement suggestions, i.e., which pairs of nodes in a given alignment $\varphi$ are appealing to repair incorrect statements replacing them by correct statements. Intuitively, we analyze which node similarities in $\varphi$ significantly deviate from the rest of the node similarities, for which we rely on mean and standard deviation. Let $\mu_\varphi$ and $\sigma_\varphi$ be the mean and standard deviation of the node similarities in $\varphi$, respectively. We establish a similarity threshold that, for all pairs whose node similarities are below such threshold, we will consider them as replacement suggestions, i.e., they significantly deviate from the rest. Therefore, we consider a pair $(u_i, \varphi(u_i))$ to be a replacement suggestion if $Sim(u_i, \varphi(u_i)) < \mu_\varphi - k \, \sigma_\varphi$, where $k \in \mathbb{R} \geq 0$. In Figure~\ref{fig:pdg-align-killer}, where \{$\varphi(u_3) = v_3$, $\varphi(u_4) = v_6$, $\varphi(u_5) = v_4$, $\varphi(u_6) = v_5$, $\varphi(u_7) = v_7$\}, we have that $\mu_\varphi=0.89$ and $\sigma_\varphi=0.04$. If we use $k=1.5$, node $u_5$ with $Sim(u_5, \varphi(u_5)) = 0.80 < 0.83$ is selected as a replacement suggestion, which corresponds to the suggestion of replacing \texttt{if (m < a[i])} by \texttt{if (m > a[i])} in the incorrect program in Figure~\ref{fig:pdg-align-killer}. We discuss the selection of $k$ below.

Second, we address the problem of finding suggestions of statements to be added or removed. Recall that we suggest statements to be added when the size of the incorrect program is less than the size of the correct program (total number of nodes). Otherwise, if the correct program is smaller than the incorrect, we suggest statements to be removed. Note that, in practice, the number of addition or removal suggestions can be large if the core of both programs are similar but they have differences in implementation. A common example in our experiments is learners who reutilize their own implementation of a console manager for reading from and writing to console. Other learners exploit utility classes to achieve the same behavior, e.g., \texttt{java.util.Scanner}. In such cases, even when the core of both programs is similar, there are a large number of non-aligned nodes that correspond to the ad-hoc console manager. If we remove such nodes, it is very unlikely that the resulting program would be correct. As a result, we only suggest nodes to be added or removed if they are directly or indirectly (one hop) connected with nodes suggested as replacements without taking direction into account. More formally, $v \in V_2 | v \notin ran \, \varphi$ is suggested as an addition or removal if $\exists u \in V_1 | (u, \varphi(u)) \in P \land |Path_U(\varphi(u), v, G_2)| \leq 1$, where $P$ is the set of replacement suggestions and $Path_U(u, v, G)$ is the shortest path between nodes $u$ and $v$ in the undirected version of graph $G$. In our example in Figure~\ref{fig:pdg-align-killer}, both $v_8$ and $v_9$ nodes are suggested to be removed since they are direct and indirect neighbors of $v_4$, which was suggested to be replaced.

Finally, we adapt edge correctness~\cite{Kuchaiev1341} ($EC$) to compute a global similarity between program dependence graphs $G_1$ and $G_2$. Edge correctness measures the number of edges that are preserved in a given approximate alignment $\varphi$, which is defined as follows:

\begin{align*}
EC(\varphi) = \dfrac{\sum\limits_{(u_i, u_j) \in E_1} IP(u_i, u_j, \varphi, E_2)}{|E_1|}
\end{align*}

\noindent where $IP(u_i, u_j, \varphi, E_2) = 1$ if and only if $(\varphi(u_i), \varphi(u_j)) \in E_2 \land l^1_e((u_i, u_j)) = l^2_e((\varphi(u_i), \varphi(u_j)))$; otherwise, $IP(u_i, u_j, \varphi, E_2) = 0$. 
